Understanding the origin of CEMP-no stars through ultra-faint dwarfs

The origin of Carbon Enhanced Metal-Poor (CEMP-no) stars with low abundances of neutron-capture elements is still unclear. These stars are ubiquitous, found primarily in the Milky Way halo and ultra-faint dwarf galaxies (UFDs). To make a major step forward, we developed a data-calibrated model for B\"ootes I that simultaneously includes all carbon sources: supernovae and asymptotic giant branch (AGB) stars both from first (Pop III) stars, and subsequent normal star formation (Pop II). We demonstrate that each of these sources leave a specific chemical signature in the gas, allowing us to identify the origin of present day CEMP-no stars through their location in the A(C)-[Fe/H] diagram. The CEMP stars with A(C)>6 are predominantly enriched by AGB Pop II stars. We identify a new class of 'moderate CEMP-s' stars with A(C)~ 7 and 0<[Ba/Fe]<+1 , imprinted by winds from AGB stars. True Pop III descendants are predicted to have A(C)<6 and a constant [C/Mg] with [Fe/H], in perfect agreement with observations in B\"ootes I and the Milky Way halo. For the first time we now have a complete picture of the origins of CEMP-no stars which can and will be verified with future observations.

==> UnderstandigTheOriginOfCEMPno (Latex)/include_tex/colors.tex <==

% workaround for colors starging with f
\makeatletter
\def\@hex@@Hex#1%
 {\if a#1A\else \if b#1B\else \if c#1C\else \if d#1D\else
  \if e#1E\else \if f#1F\else #1\fi\fi\fi\fi\fi\fi \@hex@Hex}
\makeatother

\definecolor{apcolor}{HTML}{b3003b}
\definecolor{cbcolor}{HTML}{ff0f00}
\definecolor{afcolor}{HTML}{b3443c}
\definecolor{ddcolor}{HTML}{077a2f}
\definecolor{vgcolor}{HTML}{8F00FF}

\newcommand{\AP}[1]{{\bf \color{apcolor} AP: #1}}
\newcommand{\AF}[1]{{\bf \color{afcolor} AF: #1}}
\newcommand{\VG}[1]{{\bf \color{vgcolor} VG: #1}}


==> UnderstandigTheOriginOfCEMPno (Latex)/include_tex/definizioni.tex <==
\def\be{\begin{equation}} 
\def\ee{\end{equation}} 
\def\ba{\begin{eqnarray}} 
\def\ea{\end{eqnarray}} 
\def\erfc{\rm {erfc}} 
\def\bbf{\bf} 
\def\mpc{\,{\rm {Mpc}}}
\def\mpch{\,h^{-1}{\rm {Mpc}}} 
\def\kms{\,{\rm {km\, s^{-1}}}} 
\def\cc{\,{\rm {cm^{-3}}}} 
\def\msun{{\Msun}} 
\def\vcir{{v_c}}  
\def\dt{{\Delta t}}  
\def\Gyr{{\,\rm Gyr}} 
\def\etal{{\it et al.~}}  
\def\Hm{${\rm {H^-}}\,\,$}  
%\def\HH{${\rm {H_2}}\,\,$}
\def\HH{${\rm {H_2}}$}
\def\HHp{${\rm {H_2^+}}\,\,$} 
\def\sngg{SN$_{\gamma\gamma}$~}  
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{\esc}} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HeII{\hbox{He~$\scriptstyle\rm II\ $}} 
\def\HeIII{\hbox{He~$\scriptstyle\rm III\ $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV\ $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV\ $}} 
\def\OVI{\hbox{O~$\scriptstyle\rm VI\ $}} \def\nHI{{\rm HI}} 
\def\nCIV{{\rm CIV}} \def\nOVI{{\rm OVI}} \def\nH{{\rm H}} 
\def\nHII{{\rm HII}} \def\nHe{{\rm He}} \def\nHeI{{\rm HeI}} 
\def\nHeII{{\rm HeII}} \def\nHeIII{{\rm HeIII}} \def\erg{{\rm erg}} 
\def\sr{{\rm sr}} \def\hz{{\rm Hz}} \def\cm{${\rm cm}$} 
\def\nhi{{N_{\rm HI}}} \def\sec{{\rm s}} 
\def\sigmaba{\sigma_8/usr/local/lib/tex/inputs/latex/styles} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over 
\sim \;$} \def\ltsima{$\; \buildrel < \over \sim \;$} \def\prosima{$\; 
\buildrel \propto \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} \def\la{\lsim} \def\ga{\gsim} 
\def\ie{{\frenchspacing\it i.e. }} \def\eg{{\frenchspacing\it e.g. }} 
 \def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} 
\def\la{\lsim} 
\def\ga{\gsim} 
\def\de{{\rm d}}
\def\del{\partial}
\def\zcr{Z_{\rm cr}} 
\def\ekin{\mbox{\cal E}_{\rm kin}} 
\def\ekin{{\cal E}_{\rm kin}} 
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{esc}} 
\def\Lya{Ly$\alpha$~} 
\def\sngg{SN-e$^{\pm}$~} 
\def\snggo{SN-e$^{\pm}$} 
\def\msun{\,{\rm \Msun}} 
\def\ie{{\frenchspacing\it i.e., }} 
\def\eg{{\frenchspacing\it e.g., }} 
\def\E3{{\cal E}_{\rm g}^{III}} 
\def\Eunit{\times10^{51} {\rm erg} \, \Msun^{-1}} 
\def\sEunit{10^{51} {\rm erg} \, \Msun^{-1}} 
\def\ozs{\Omega_Z^{sfh}} 
\def\ozo{\Omega_Z^{obs}} 
\def\Onot{\Omega_0} 
\def\Msun{\rm M_\odot}
\def\Zsun{\rm Z_\odot}
\def\rvir{r_{vir}}
\def\rvir{r_{vir}}
\def\vvir{v_{vir}} 
\def\mvir{M_{vir}} 
\def\Tvir{T_{vir}} 
\def\r12{r_{1/2}} 
\def\x12{x_{1/2}} 
\def\v12{v_{1/2}}
\def\ftd{F_{T,D}}
\def\Msf{M_{sf}}



% element astro-like
\def\HI{\hbox{H~$\scriptstyle\rm I $~}}
\def\HII{\hbox{H~$\scriptstyle\rm II $~}}
\def\HeI{\hbox{He~$\scriptstyle\rm I $~}}
\def\HeII{\hbox{He~$\scriptstyle\rm II $~}}
\def\HeIII{\hbox{He~$\scriptstyle\rm III $~}}
%
%\def\CIIion{\hbox{C~$\scriptstyle\rm II $}}
%\def\OIion{\hbox{O~$\scriptstyle\rm I $}}
%\def\OIIIion{\hbox{O~$\scriptstyle\rm III $}}
%\def\NIIion{\hbox{O~$\scriptstyle\rm II $}}
%
\def\CIIion{${\rm C}^{+}$}
\def\OIIIion{${\rm O}^{++}$}
\def\NIIion{${\rm N}^{+}$}

% FIR emission lines
\def\CII{\hbox{[C~$\scriptstyle\rm II $]}}
\def\OI{\hbox{[O~$\scriptstyle\rm I $]}} 
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]}} 
\def\NII{\hbox{[N~$\scriptstyle\rm II $]}}

% absorption lines
\def\MGII{\hbox{Mg~$\scriptstyle\rm II $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV $}}
\def\SiI{\hbox{Si~$\scriptstyle\rm I $}}
\def\SII{\hbox{Si~$\scriptstyle\rm II $}} 
\def\NIIa{\hbox{N~$\scriptstyle\rm IIa $}} 

\def\red{\color{red}}
\def\green{\color{green}}
\def\cyan{\color{cyan}}

% mnras style for code names
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand{\quotes}[1]{``#1''}
\newcommand{\quotesing}[1]{`#1'}

% cosmo
\def\vir{\rm vir}
\def\halo{\rm h}
\def\cent{\rm c}
\def\rvir{r_{\vir}}
\def\zlos{\langle Z\rangle}
%
\def\diinu{\Delta I_{\nu}\slash I_{\nu}}
\def\diiDnu{\Delta I\slash I}
\def\mujb{\mu {\rm Jy}/{\rm beam}}

% math
\def\gt{$>$}

% chemistry
\def\nh2{n_{\rm H2}}
\def\fh2{f_{\rm H2}}
\def\fhp{f_{\rm H+}}
\def\Hp{${\rm H}^{+}$}
\def\dust{\mathcal{D}}
\def\mp{m_{\rm p}}

% units
\def\arcsec{^{\prime\prime}}
\def\angstrom{\textrm{A\kern -1.3ex\raisebox{0.6ex}{$^\circ$}}}
\def\myr{\rm Myr}
\def\mum{\mu{\rm m}}
% solar stuff
\def\msun{{\rm M}_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{\dust_{\odot}}
%
\def\cc{{\rm cm}^{-3}}
\def\colcm{{\rm cm}^{-2}}
%
\def\msunyr{\msun\,{\rm yr}^{-1}}
\def\surfd{\msun\,{\rm kpc}^{-2}}
\def\surfsfr{\msun\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\def\surfdpc{\msun\,{\rm pc}^{-2}}
\def\surfl{\lsun\,{\rm kpc}^{-2}}
\def\voldpc{\msun\,{\rm pc}^{-3}}
%
\def\kpc{{\rm kpc}}
\def\SFR{{\rm SFR}}

%lum and ions
\def\SCII{\Sigma_{\rm [CII]}}
\def\SOIII{\Sigma_{\rm [OIII]}}
\def\SNII{\Sigma_{\rm [NII]}}
\def\SigmaCII{\Sigma_{\rm C+}}
\def\SigmaOIII{\Sigma_{\rm O++}}
\def\SigmaNII{\Sigma_{\rm N+}}
% additional convenience stuff
\def\sigmasfr{\dot{\Sigma}_{\star}}

% names shortcuts
\def\althaea{Alth{\ae}a}
\def\highz{$\mbox{high-}z$~}

==> UnderstandigTheOriginOfCEMPno (Latex)/include_tex/journals.tex <==
\def\amp{\&}
\def\nat{Nature}
\def\na{New Astronomy}
\def\pra{Phys. Rev. A}
\def\prb{Phys. Rev. B}
\def\prc{Phys. Rev. B}
\def\prd{Phys. Rev. D}
\def\mnras{MNRAS}
\def\apj{ApJ}
\def\apjl{ApJL}
\def\apjs{ApJS}
\def\aap{A\&A}
\def\aaps{A\&A Supp.}
\def\aapr{A\&A Rev.}
\def\araa{ARA\&A}
\def\aj{AJ}
\def\qjras{QJRAS}
\def\physrep{Phys. Rep.}
\def\apss{Ap\&SS}               % Astrophysics and Space Science
\def\planss{P\&SS}              % Planetary and Space Science
\def\pasa{Publ. Astr. Soc. Australia}
\def\pasp{Publ. Astr. Soc. Pac.}
\def\jcp{J. Chem. Phys.}
\def\pasj{Pub. Astron. Soc. Japan}
\def\ssr{Space Science Reviews}
\def\grl{Geophysical Research Letters}
\def\jgr{Journal of Geophysical Research}
\def\nar{New Astronomy Reviews}
\def\jcap{JCAP}
\def\fcp{Fundamentals of Cosmic Physics}



==> UnderstandigTheOriginOfCEMPno (Latex)/include_tex/pacchetti.tex <==
\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage[normalem]{ulem}

\usepackage{verbatim}

\usepackage{color}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{epstopdf}

\usepackage{url}
\usepackage{xcolor}


==> include_tex/colors.tex <==

% workaround for colors starging with f
\makeatletter
\def\@hex@@Hex#1%
 {\if a#1A\else \if b#1B\else \if c#1C\else \if d#1D\else
  \if e#1E\else \if f#1F\else #1\fi\fi\fi\fi\fi\fi \@hex@Hex}
\makeatother

\definecolor{apcolor}{HTML}{b3003b}
\definecolor{cbcolor}{HTML}{ff0f00}
\definecolor{afcolor}{HTML}{b3443c}
\definecolor{ddcolor}{HTML}{077a2f}
\definecolor{vgcolor}{HTML}{8F00FF}

\newcommand{\AP}[1]{{\bf \color{apcolor} AP: #1}}
\newcommand{\AF}[1]{{\bf \color{afcolor} AF: #1}}
\newcommand{\VG}[1]{{\bf \color{vgcolor} VG: #1}}


==> include_tex/definizioni.tex <==
\def\be{\begin{equation}} 
\def\ee{\end{equation}} 
\def\ba{\begin{eqnarray}} 
\def\ea{\end{eqnarray}} 
\def\erfc{\rm {erfc}} 
\def\bbf{\bf} 
\def\mpc{\,{\rm {Mpc}}}
\def\mpch{\,h^{-1}{\rm {Mpc}}} 
\def\kms{\,{\rm {km\, s^{-1}}}} 
\def\cc{\,{\rm {cm^{-3}}}} 
\def\msun{{\Msun}} 
\def\vcir{{v_c}}  
\def\dt{{\Delta t}}  
\def\Gyr{{\,\rm Gyr}} 
\def\etal{{\it et al.~}}  
\def\Hm{${\rm {H^-}}\,\,$}  
%\def\HH{${\rm {H_2}}\,\,$}
\def\HH{${\rm {H_2}}$}
\def\HHp{${\rm {H_2^+}}\,\,$} 
\def\sngg{SN$_{\gamma\gamma}$~}  
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{\esc}} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HeII{\hbox{He~$\scriptstyle\rm II\ $}} 
\def\HeIII{\hbox{He~$\scriptstyle\rm III\ $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV\ $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV\ $}} 
\def\OVI{\hbox{O~$\scriptstyle\rm VI\ $}} \def\nHI{{\rm HI}} 
\def\nCIV{{\rm CIV}} \def\nOVI{{\rm OVI}} \def\nH{{\rm H}} 
\def\nHII{{\rm HII}} \def\nHe{{\rm He}} \def\nHeI{{\rm HeI}} 
\def\nHeII{{\rm HeII}} \def\nHeIII{{\rm HeIII}} \def\erg{{\rm erg}} 
\def\sr{{\rm sr}} \def\hz{{\rm Hz}} \def\cm{${\rm cm}$} 
\def\nhi{{N_{\rm HI}}} \def\sec{{\rm s}} 
\def\sigmaba{\sigma_8/usr/local/lib/tex/inputs/latex/styles} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over 
\sim \;$} \def\ltsima{$\; \buildrel < \over \sim \;$} \def\prosima{$\; 
\buildrel \propto \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} \def\la{\lsim} \def\ga{\gsim} 
\def\ie{{\frenchspacing\it i.e. }} \def\eg{{\frenchspacing\it e.g. }} 
 \def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} 
\def\la{\lsim} 
\def\ga{\gsim} 
\def\de{{\rm d}}
\def\del{\partial}
\def\zcr{Z_{\rm cr}} 
\def\ekin{\mbox{\cal E}_{\rm kin}} 
\def\ekin{{\cal E}_{\rm kin}} 
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{esc}} 
\def\Lya{Ly$\alpha$~} 
\def\sngg{SN-e$^{\pm}$~} 
\def\snggo{SN-e$^{\pm}$} 
\def\msun{\,{\rm \Msun}} 
\def\ie{{\frenchspacing\it i.e., }} 
\def\eg{{\frenchspacing\it e.g., }} 
\def\E3{{\cal E}_{\rm g}^{III}} 
\def\Eunit{\times10^{51} {\rm erg} \, \Msun^{-1}} 
\def\sEunit{10^{51} {\rm erg} \, \Msun^{-1}} 
\def\ozs{\Omega_Z^{sfh}} 
\def\ozo{\Omega_Z^{obs}} 
\def\Onot{\Omega_0} 
\def\Msun{\rm M_\odot}
\def\Zsun{\rm Z_\odot}
\def\rvir{r_{vir}}
\def\rvir{r_{vir}}
\def\vvir{v_{vir}} 
\def\mvir{M_{vir}} 
\def\Tvir{T_{vir}} 
\def\r12{r_{1/2}} 
\def\x12{x_{1/2}} 
\def\v12{v_{1/2}}
\def\ftd{F_{T,D}}
\def\Msf{M_{sf}}



% element astro-like
\def\HI{\hbox{H~$\scriptstyle\rm I $~}}
\def\HII{\hbox{H~$\scriptstyle\rm II $~}}
\def\HeI{\hbox{He~$\scriptstyle\rm I $~}}
\def\HeII{\hbox{He~$\scriptstyle\rm II $~}}
\def\HeIII{\hbox{He~$\scriptstyle\rm III $~}}
%
%\def\CIIion{\hbox{C~$\scriptstyle\rm II $}}
%\def\OIion{\hbox{O~$\scriptstyle\rm I $}}
%\def\OIIIion{\hbox{O~$\scriptstyle\rm III $}}
%\def\NIIion{\hbox{O~$\scriptstyle\rm II $}}
%
\def\CIIion{${\rm C}^{+}$}
\def\OIIIion{${\rm O}^{++}$}
\def\NIIion{${\rm N}^{+}$}

% FIR emission lines
\def\CII{\hbox{[C~$\scriptstyle\rm II $]}}
\def\OI{\hbox{[O~$\scriptstyle\rm I $]}} 
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]}} 
\def\NII{\hbox{[N~$\scriptstyle\rm II $]}}

% absorption lines
\def\MGII{\hbox{Mg~$\scriptstyle\rm II $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV $}}
\def\SiI{\hbox{Si~$\scriptstyle\rm I $}}
\def\SII{\hbox{Si~$\scriptstyle\rm II $}} 
\def\NIIa{\hbox{N~$\scriptstyle\rm IIa $}} 

\def\red{\color{red}}
\def\green{\color{green}}
\def\cyan{\color{cyan}}

% mnras style for code names
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand{\quotes}[1]{``#1''}
\newcommand{\quotesing}[1]{`#1'}

% cosmo
\def\vir{\rm vir}
\def\halo{\rm h}
\def\cent{\rm c}
\def\rvir{r_{\vir}}
\def\zlos{\langle Z\rangle}
%
\def\diinu{\Delta I_{\nu}\slash I_{\nu}}
\def\diiDnu{\Delta I\slash I}
\def\mujb{\mu {\rm Jy}/{\rm beam}}

% math
\def\gt{$>$}

% chemistry
\def\nh2{n_{\rm H2}}
\def\fh2{f_{\rm H2}}
\def\fhp{f_{\rm H+}}
\def\Hp{${\rm H}^{+}$}
\def\dust{\mathcal{D}}
\def\mp{m_{\rm p}}

% units
\def\arcsec{^{\prime\prime}}
\def\angstrom{\textrm{A\kern -1.3ex\raisebox{0.6ex}{$^\circ$}}}
\def\myr{\rm Myr}
\def\mum{\mu{\rm m}}
% solar stuff
\def\msun{{\rm M}_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{\dust_{\odot}}
%
\def\cc{{\rm cm}^{-3}}
\def\colcm{{\rm cm}^{-2}}
%
\def\msunyr{\msun\,{\rm yr}^{-1}}
\def\surfd{\msun\,{\rm kpc}^{-2}}
\def\surfsfr{\msun\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\def\surfdpc{\msun\,{\rm pc}^{-2}}
\def\surfl{\lsun\,{\rm kpc}^{-2}}
\def\voldpc{\msun\,{\rm pc}^{-3}}
%
\def\kpc{{\rm kpc}}
\def\SFR{{\rm SFR}}

%lum and ions
\def\SCII{\Sigma_{\rm [CII]}}
\def\SOIII{\Sigma_{\rm [OIII]}}
\def\SNII{\Sigma_{\rm [NII]}}
\def\SigmaCII{\Sigma_{\rm C+}}
\def\SigmaOIII{\Sigma_{\rm O++}}
\def\SigmaNII{\Sigma_{\rm N+}}
% additional convenience stuff
\def\sigmasfr{\dot{\Sigma}_{\star}}

% names shortcuts
\def\althaea{Alth{\ae}a}
\def\highz{$\mbox{high-}z$~}
